Almost prime values of the order of abelian varieties over finite fields

Let $E/\mathbb Q$ be an elliptic curve, and denote by $N(p)$ the number of $\mathbb{F}_p$-points of the reduction modulo $p$ of $E$. A conjecture of Koblitz, refined by Zywina, states that the number of primes $p \leq X$ at which $N(p)$ is also prime is asymptotic to $C_E \cdot X / \log(X)^2$, where $C_E$ is an arithmetically-defined non-negative constant. Following Miri-Murty (2001) and others, Y.R. Liu (2006) and David-Wu (2012) study the number of prime factors of $N(p)$. We generalize their arguments to abelian varieties $A / \mathbb Q$ whose adelic Galois representation has open image in $\textrm{GSp}_{2g} \widehat{\mathbb Z}$. Our main result, after David-Wu, finds a conditional lower bound on the number of primes at which $\# A_p ( \mathbb{F}_p)$ has few prime factors. We also present some experimental evidence in favor of a generalization of Koblitz's conjecture to this context.

==> BibFiles/BibTemplates.tex <==
%%%  see https://verbosus.com/bibtex-style-examples.html  %%%

%%% use note = {} to include the LABEL in the bibliography, to get a useful reference page 
%%% comment out "\AtEveryBibitem{\clearfield{note}}" on CustomCommands.tex to get back to a usual bibliography

@article{,
note = {},
journal = {},
number = {},
pages = {},
title = {},
author = {},
volume = {},
year = {},
}
%%%%%%%%%%%%%%%%%%%%%
@book{,
note = {},
author = {}, 
title  = {},
publisher = {},
year      = {},
volume    = {},
series    = {},
edition   = {},
}
%%%%%%%%%%%%%%%%%%%%%%
@phdthesis{,
note = {},
author = {}, 
title = {},
school = {},
year = {},
}
%%%%%%%%%%%%%%%%%%
@proceedings{,
note = {},
title = {},
year = {},
editor = {},
volume = {},
series = {},
organization = {},
publisher = {},
}
%%%%%%%%%%%%%%%%5
@incollection{ ,
author = {},
title = {},
editor = {},
booktitle = {},
publisher = {},
address = {},
year = {},
pages = {}
}
